MAP-REDUCE Runtime Enforcement of Information Flow Policies

We propose a flexible framework that can be easily customized to enforce a large variety of information flow properties. Our framework combines the ideas of secure multi-execution and map-reduce computations. The information flow property of choice can be obtained by simply changes to a map (or reduce) program that control parallel executions. We present the architecture of the enforcement mechanism and its customizations for non-interference (NI) (from Devriese and Piessens) and some properties proposed by Mantel, such as removal of inputs (RI) and deletion of inputs (DI), and demonstrate formally soundness and precision of enforcement for these properties.

==> DI-Example-IO.tex <==
\begin{lrbox}{\mylistingbox}%
\begin{tabular}{l}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\hspace{3pt}
\begin{minipage}{130pt}
The input to \MAP:\\
\emph{(The last input item is not consumed.)} 
\begin{tabular}{|c|c|c|c|c|}
	\hline
	Time & 0 & 1 & 2 & 3 \\
    \hline
	\linecode{cH1} & $\VTRUE$ & \NIL & \NIL & \NIL\\
	\hline
	\linecode{cH2} & \NIL & \NIL & \NIL & $M$ \\
	\hline
	\linecode{cL1} & \NIL & \VFALSE & \NIL & \NIL\\
	\hline
	\linecode{cL2} & \NIL & \NIL & $m$ & \NIL\\
	\hline 
\end{tabular} \\
\end{minipage} $\Longrightarrow$ \MAP \\
%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{minipage}{110pt}
%\centering
%~\\
%$\Downarrow$
%\end{minipage} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Local Executions: \\
\begin{tabular}{|l|}
\hline
The high execution \Progl{0}:\\
\begin{tabular}{p{110pt}p{180pt}}
The local input: & The local output:\\
\begin{tabular}{|c|c|c|c|c|}
	\hline
	\linecode{cH1} & $\VTRUE$ & \NIL & \NIL \\
	\hline
	\linecode{cH2} & \NIL & \NIL & \NIL \\
	\hline
	\linecode{cL1} & \NIL & \VFALSE & \NIL \\
	\hline
	\linecode{cL2} & \NIL & \NIL & $m$ \\
	\hline
\end{tabular} & 
\begin{minipage}{180pt}
\begin{tabular}{|c|c|c|c|c|>{\centering\arraybackslash}p{25pt}|>{\centering\arraybackslash}p{25pt}|}
	\hline	
	\linecode{cH3} & \NIL & \NIL & \NIL & \NIL & $m$ & \NIL\\
	\hline
	\linecode{cL3} & \NIL & \NIL & \NIL & \NIL &  \NIL & $m$\\
	\hline 	
\end{tabular}
\vspace{25pt}
\end{minipage} \\

\end{tabular} \\\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%The second execution
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline
The low execution \Progl{1}:\\
\begin{tabular}{p{110pt}p{105pt}}
The local input: & The local output:\\
\begin{tabular}{|c|c|c|c|c|}
	\hline
	\linecode{cH1} & $\VFALSE$ & \NIL & \NIL & \NIL\\
	\hline
	\linecode{cH2} & \NIL & \NIL & \NIL & $*$\\
	\hline
	\linecode{cL1} & \NIL & \VFALSE & \NIL & \NIL\\
	\hline
	\linecode{cL2} & \NIL & \NIL & $m$ & \NIL\\
	\hline
\end{tabular} &
\begin{minipage}{180pt}
\begin{tabular}{|c|c|c|c|c|>{\centering\arraybackslash}p{25pt}|>{\centering\arraybackslash}p{25pt}|}
	\hline	
	\linecode{cH3} & \NIL & \NIL & \NIL & \NIL & $* + m$ & \NIL\\
	\hline
	\linecode{cL3} & \NIL & \NIL & \NIL & \NIL & \NIL & $* + m$\\
	\hline
\end{tabular}
\vspace{24pt}
\end{minipage}
%\\~
\end{tabular} \\\\ \hline
The other execution \Progl{2}:\\
\begin{tabular}{p{110pt}p{105pt}}
The local input: & The local output:\\
\begin{tabular}{|c|c|c|c|c|}
	\hline
	\linecode{cH1} & $\VFALSE$ & \NIL & \NIL & \NIL\\
	\hline
	\linecode{cH2} & \NIL & \NIL & \NIL & $*$\\
	\hline
	\linecode{cL1} & \NIL & \VFALSE & \NIL & \NIL\\
	\hline
	\linecode{cL2} & \NIL & \NIL & $m$ & \NIL\\
	\hline
\end{tabular} &
\begin{minipage}{105pt}
\begin{tabular}{|c|c|c|c|c|>{\centering\arraybackslash}p{25pt}|>{\centering\arraybackslash}p{25pt}|}
	\hline	
	\linecode{cH3} & \NIL & \NIL & \NIL & \NIL & $* + m$ & \NIL\\
	\hline
	\linecode{cL3} & \NIL & \NIL & \NIL & \NIL & \NIL & $* + m$\\
	\hline
\end{tabular}
\vspace{24pt}
\end{minipage}
%\\~
\end{tabular} \\\\ \hline

\end{tabular}  \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%   END LOCAL EXECUTION%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%% BEGIN OUTPUT%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\hspace{139pt}
%\begin{minipage}{180pt}
%\centering
%~\\
%$\Downarrow$\\
%\end{minipage} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{3pt}
\hspace{70pt}
\REDUCE\ $\Longrightarrow$ 
\begin{minipage}{180pt}
~\\
The output by \REDUCE:\\
\begin{tabular}{|c|c|c|c|c|>{\centering\arraybackslash}p{25pt}|>{\centering\arraybackslash}p{25pt}|}
	\hline
	Time & 0 & 1 & 2 & 3 & 4 & 5 \\
	\hline	
	\linecode{cH3} & \NIL & \NIL & \NIL & \NIL & $m$ & \NIL\\
	\hline
	\linecode{cL3} & \NIL & \NIL & \NIL & \NIL & \NIL & $* + m$\\
	\hline
\end{tabular}
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}
\end{lrbox}







%\begin{tabular}{ll}
%The input to \MAP:  & \\
%\begin{tabular}{|c|c|c|c|c|}
%    \hline
%	\linecode{cH1} & $\VTRUE$ & \NIL & \NIL & \NIL\\
%	\hline
%	\linecode{cH2} & \NIL & \NIL & \NIL & $M$\\
%	\hline
%	\linecode{cL1} & \NIL & \VFALSE & \NIL & \NIL \\
%	\hline
%	\linecode{cL2} & \NIL & \NIL & $m$ & \NIL\\
%	\hline 
%\end{tabular} & $\Longrightarrow$ \\
%\begin{minipage}{100pt}
%\emph{(The last input item is not consumed)}
%\end{minipage}\\
%\vspace{130pt}\\
%The output by \REDUCE: ~ \\
%\begin{tabular}{|c|c|c|c|c|c|}
%	\hline	
%	\linecode{cH3} & \NIL & \NIL & \NIL & $m$ & \NIL\\
%	\hline
%	\linecode{cL3} & \NIL & \NIL & \NIL & \NIL & $* + m$\\
%	\hline
%\end{tabular} & $\Longrightarrow$ 
%\end{tabular} &

==> NI-Example-TMTR.tex <==
\subfloat[Configuration of \TAV]{
\label{fig:table:NI:MAP:example}
\begin{minipage}{0.4\columnwidth}
\centering
\begin{tabular}{|c|c|c|}
\hline
~ & \tindex{0} & \tindex{1} \\
\hline
\linecode{cH1} & \tgetask & \task \\
\hline
\linecode{cH2} & \tgetask & \task \\
\hline
\linecode{cL1} & \tget & \tgetask \\
\hline
\linecode{cL2} & \tget & \tgetask \\
\hline
\end{tabular}
\end{minipage}
} \hfill
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subfloat[Configuration of \TPV]{
\label{fig:table:NI:REDUCE:example}
\begin{minipage}{0.4\columnwidth}
\centering
\vspace{25pt}
\begin{tabular}{|c|c|c|}
\hline
~ &  \tindex{0} & \tindex{1} \\
\hline
\linecode{cH3} & \ttellput & \tnoaction \\
\hline
\linecode{cL3} & \tnoaction & \ttellput \\
\hline
\end{tabular}
\end{minipage}
}
